Supporting Hard Queries over Probabilistic Preferences

Preference analysis is widely applied in various domains such as social choice and e-commerce. A recently proposed framework augments the relational database with a preference relation that represents uncertain preferences in the form of statistical ranking models, and provides methods to evaluate Conjunctive Queries (CQs) that express preferences among item attributes. In this paper, we explore the evaluation of queries that are more general and harder to compute. The main focus of this paper is on a class of CQs that cannot be evaluated by previous work. These queries are provably hard since relate variables that represent items being compared. To overcome this hardness, we instantiate these variables with their domain values, rewrite hard CQs as unions of such instantiated queries, and develop several exact and approximate solvers to evaluate these unions of queries. We demonstrate that exact solvers that target specific common kinds of queries are far more efficient than general solvers. Further, we demonstrate that sophisticated approximate solvers making use of importance sampling can be orders of magnitude more efficient than exact solvers, while showing good accuracy. In addition to supporting provably hard CQs, we also present methods to evaluate an important family of count queries, and of top-k queries.

==> tex/backup.tex <==
\textbf{Previous works.} 

In an early vision paper, Jacob et al. proposed a novel relation designed for pairwise preferences to augment traditional RDBMS~\cite{DBLP:journals/pvldb/JacobKS14}. An instance of this preference relation contains preference pairs grouped into sessions. The tuples are in the form of $(s;l;r)$ where $s$ is the session identifier and $s$ prefers item $l$ to item $r$. For example, in a database of presidential election polls, a tuple $(\val{Dave},\val{Oct-5};\val{Sanders};\val{Rubio})$ denotes that on October $5^{th}$ Dave preferred Sanders to Rubio. Here, $(\val{Dave},\val{Oct-5})$ is the session identifier. This preference relation supports various operations, e.g., transitive closure, preference clustering.

Then we embarked on the challenge of preferences being incomplete or uncertain. Mallows model~\cite{Mallows1957} particularly draws our attention. We developed a workload-driven approach to model uncertain preferences with Mallows mixtures~\cite{DBLP:conf/webdb/StoyanovichIP16}.

Then we extended the preference database in the early vision paper~\cite{DBLP:journals/pvldb/JacobKS14} and proposed RIM-PPD that is short for RIM-based Probabilistic Preference Database~\cite{DBLP:conf/pods/KenigKPS17}. Repeated Insertion Model (RIM) is a generative ranking model giving rise to a family of ranking models including Mallows. In RIM-PPD, each preference session is associated with a RIM model, i.e., a distribution of rankings. And all sessions are assumed to be independent from each other.

We also developed a query engine for Conjunctive Queries (CQ) that are \textit{itemwise}~\cite{DBLP:conf/sigmod/CohenKPKS18}. 

Assume $\qOneIntro$ is true over the three sessions in Figure~\ref{fig:elections} with probabilities $\{p_1, p_2, p_3\}$, respectively. Since all sessions are independent, the answer to $\qOneIntro$ is $1 - (1-p_1)(1-p_2)(1-p_3)$, i.e., at least one session supports $\qOneIntro$.

Now the problem is calculating $p_i, 1 \leq i \leq 3$, the probability of $\qOneIntro$ over a particular session that has a particular RIM model. The semantics of $p_i$ is the expectation that a ranking $\btau$ sampled from the RIM model satisfies $\qOneIntro$. Note that $\qOneIntro$ can be represented by a \textit{label pattern} --- a partial order of labels. A \textit{label} is a value of an attribute of an item, e.g., gender (attribute) of $l$ (item) is $F$ (label). The corresponding label pattern is $F \succ M$, so $\qOneIntro$ essentially asks the preferences over labels $F$ and $M$. Given a ranking $\btau$ and a label $L$, a \textit{matching} item $\tau$ of $L$ is an item with label $L$ in $\btau$. The sets of potential matching items for $F$ and $M$ are $S_F = \{\mathtt{Clinton}\}$ and $S_M = \{\mathtt{Trump}, \mathtt{Sanders}, \mathtt{Rubio}\}$. A ranking $\btau$ satisfies $l \succ r$ if there exist a matching item $\tau_l \in S_F$ for $l$ and a matching item $\tau_r \in S_M$ for $r$ s.t. $\tau_l \succ \tau_r$ by $\btau$. This is known as the \textit{label matching} semantics. The expectation of a label pattern over a RIM model is a novel inference problem. We solved it with LTM algorithm~\cite{DBLP:conf/sigmod/CohenKPKS18}.


\section{Special queries}

We've been focusing on non-itemwise CQ evaluation. RIM-PPD can also support two operators over a query $Q$.

\subsection{Count}

A non-itemwise CQ $Q$ asks whether there exists a session that supports $Q$. By applying the count operator, $\countq(Q)$ calculates the number of sessions satisfying $Q$. Since RIM-PPD is probabilistic. The value of $\countq(Q)$ is also under the \textit{Possible World Semantics}, i.e., what the is expectation of $\countq(Q)$ over the distribution of Possible Worlds. 

Let $S = \{ s_1, \ldots, s_n\}$ denote the $n$ sessions in p-relation. Since these sessions are assumed to be independent, the expectation of $\countq(Q)$ is the sum of the probabilities that the sessions satisfy $Q$.

\[
\countq(Q) = \sum_{i=1}^{n} Pr(Q|s_i)
\]

\subsection{Top-K}

This operator is similar to the top-$K$ optimization in our previous paper~\cite{DBLP:conf/sigmod/CohenKPKS18}. Given a query $Q$ and an integer $K$, $\topk(Q, K)$ finds the $K$ most supportive sessions, i.e., the ones that satisfy $Q$ with the highest probabilities.

We implement two strategies for this operator. This first strategy calculates the probability of satisfying $Q$ for each session, then selects $K$ most supportive sessions. The second strategy first quickly calculates the upper bounds of all sessions, then calculates the exact probability of sessions in descending order of their upper bounds, and stops once there are $K$ sessions with exact probabilities greater than the exact probabilities or upper bounds of rest sessions.

Evaluating query $Q$ over a session is an inference problem of a pattern union $G$ over the RIM model $\RIM(\bsigma, \Pi)$ of this session. Section~\ref{sec:approx:ub} has presented an approach to compute upper bound of any pattern union using bipartite solver. Here, we use the a similar technique to construct a new pattern union $G'$ by calculating transitive closure of patterns in $G$ and removing some labels and edges.

Since we are removing labels and edges here, we want to preserve the edges that are the hardest to satisfy, thus $G'$ ends up with tighter upper bound. Recall the definition of $\alpha(l)$ and $\beta(l)$ meaning the position of the best ranked item and worst ranked item with label $l$ in a permutation. The ease of an edge $(l, r)$ being satisfied by a random permutation from $\RIM(\bsigma, \Pi)$ is estimated by:

\[
\mathtt{ease}(l, r | \bsigma) = \alpha( l| \bsigma) - \beta( r| \bsigma)
\]

We construct $G'$ with edges of small $\mathtt{ease}$ values. If only one edge is selected for each pattern, $G'$ is a union of two-label patterns, and $\topk(Q, K)$ invokes two-label solver accordingly. Otherwise, $G'$ is union of bipartite patterns, then bipartite solver will be invoked.

Exact solvers have complexity exponential with number of labels, so $G'$ is much faster to compute. And less labels and edges gives less constraints, so more permutations can satisfy $G'$, i.e., $Pr(G'|\bsigma, \Pi) \geq Pr(G|\bsigma, \Pi)$.

\haoyue{It is still missing that a pre-processing step about whether the speedup of top-k is enough. But this may be unnecessary. Since the issue is due to the system implementation (e.g., using Python, the overhead time of multi-processing module). From the perspective of algorithm, the speedup still holds theoretically.}
